Data Market Platforms: Trading Data Assets to Solve Data Problems

Data only generates value for a few organizations with expertise and resources to make data shareable, discoverable, and easy to integrate. Sharing data that is easy to discover and integrate is hard because data owners lack information (who needs what data) and they do not have incentives to prepare the data in a way that is easy to consume by others. In this paper, we propose data market platforms to address the lack of information and incentives and tackle the problems of data sharing, discovery, and integration. In a data market platform, data owners want to share data because they will be rewarded if they do so. Consumers are encouraged to share their data needs because the market will solve the discovery and integration problem for them in exchange for some form of currency. We consider internal markets that operate within organizations to bring down data silos, as well as external markets that operate across organizations to increase the value of data for everybody. We outline a research agenda that revolves around two problems. The problem of market design, or how to design rules that lead to the outcomes we want, and the systems problem, how to implement the market and enforce the rules. Treating data as a first-class asset is sorely needed to extend the value of data to more organizations, and we propose data market platforms as one mechanism to achieve this goal.

==> sections/datavalue.tex <==
\section{The Value of Data}
\label{sec:datavalue}

\notera{macro, micro, subscription, coase?}
\notera{business value, extrinsic vs intrinsic}

What's the value of data? This question has kept academics and practitioners in
economics, law, business, computer science and other disciplines
busy.~\cite{varian1, valuedata1, imf}. Answering the question in its full
generality is outside the scope of this paper. Instead, we focus on the narrower
yet difficult goal of choosing a price that satisfies sellers and buyers.

The crux of the problem is that the value of a dataset may be different for a
seller and a prospective buyer. Sellers may choose to price their datasets based
on the effort they spent in acquiring and preparing the data, for example.
Buyers may be willing to pay for a dataset based on the expectation of profit
the dataset may bring them: \eg how much they will improve a process and how
valuable that is. None of these strategies is guaranteed to converge to a
price---and hence a transaction agreement---between participants. 

And yet, this is how prices are set in current markets of datasets such as
Dawex~\cite{dawex}, Snowflake's Data Exchange~\cite{snowflake-exchange}, and
many others.  Sellers choose a fixed price for datasets without knowing what the
demand is and buyers who are willing to pay that price obtain the datasets,
without knowing how useful the dataset will be to solve their problem. This
leaves both sellers and buyers unsatisfied. Buyers may pay a high price for
datasets that do not yield the expected results. Similarly, sellers may
undervalue datasets that could yield more profits because they lack information
about what buyers want.

A tempting option to the database community is to value datasets based on their
intrinsic properties, such as quality, freshness, whether they include
provenance information or not, etc. Unfortunately, valuing datasets based on the
intrinsic properties of data \emph{alone} does not work either. We illustrate
why with the following scenarios:

\textit{\textbf{Example 1:} Two datasets A and B contain the same number of
records and cover the same domain. The only difference is that while A is
missing 1\% of its values, B is missing 30\% of them. Which dataset is more
valuable?  Intuition says the first dataset because of the fewer missing values
it contains.}

However, if the desired answer involves a set of values that appear in B, but
not in A, then B may be more valuable for this particular task, even though A
has fewer missing values.

\textit{\textbf{Example 2:} Consider two datasets that contain crime data of the
city of Chicago.  The first one is a snapshot of 12/31/2010. The second one is a
current up-to-date snapshot. Which one is more valuable in this case?}

Freshness is usually a positive trait of a dataset. However, if I’m trying to
understand what the crime in Chicago was in 2010 -- for example, before a
particular political event -- then the snapshot from 2010 will be more valuable
than the current one.

\textit{\textbf{Example 3:} We want to predict a variable of interest, X. We
have a dataset with 5 features and a second dataset with 20 features that
subsumes the first. Would you pay more money for the second dataset than for the
first?}

Even though more features may seem better, if the dataset with 5 features is
good enough to predict the variable of interest, adding more features may not
help at all -- in which case paying more for such a dataset would be pointless. In
fact, adding more features may lead to overfitting the model, hence achieving
worse quality. This would then require doing feature engineering, therefore
consuming more of the buyer’s resources. In this last case, one would pay
more for the first dataset, since it’s the one that helps solve the task at hand
better.

So, if intrinsic properties of data are not a good proxy to value it, what
is?

\subsubsection*{Intrinsic vs Extrinsic Value of Data}

In the markets we envision, the value (and price) of a dataset is decided by the
arbiter based on the economic principles of supply and
demand~\cite{supplyanddemand}. A scarce dataset that lots of buyers want will be
priced higher than a common dataset that is hardly ever requested, regardless of
the intrinsic properties of such datasets. In other words, the value of a
dataset is primarily extrinsic. 

\mypar{The role of intrinsic properties} When intrinsic properties of datasets
are important to buyers, they can explicitly let the arbiter know. If, as a
consequence of buyers' requests, a demand is created for a particular dataset
with, say, few missing values, sellers who provide those datasets will profit
more.

In conclusion, we argue that the value of a dataset should be established by the
market as a function of supply and demand and that when intrinsic properties of
a dataset are valuable, buyers will declare such is the case as part of the
request generated by data buyers. 

Having discussed how to price data we now dive into the market design component
of our vision.


